Transport and hydrodynamic calculations of direct photons at FAIR

The microscopic transport model UrQMD and a micro+macro hybrid model are used to calculate direct photon spectra from U+U-collisions at Elab = 35 AGeV as will be measured by the CBM-collaboration at FAIR. In the hybrid model, the intermediate high-density part of the nuclear interaction is described with ideal 3+1-dimensional hydrodynamics. Different equations of state of the matter created in the heavy-ion collisions are investigated and the resulting spectra of direct photons are predicted. The emission patterns of direct photons in space and time are discussed.

==> v2.tex <==
%# cascade Cbm35_cen_ca_spectrum.v2.stat
%# cheos Cbm35_cen_xi_spectrum.v2.stat
%# hgeos Cbm35_cen_hg_spectrum.v2.stat
%# bmeos Cbm35_cen_qg_spectrum.v2.stat
%#%: hgeos 
%#number of gammas: 4027.905908
%#events 2000 lines 90001020
%#V DICE 0x4c2fe249
%#V DICE 0x4c2fdf7b
%#%: hgeos bmeos cheos 
%#average: v2
%#V hydrophotons master v1.4-14-g9842687M
%#V UrQMD master u3.3p1-67-g887a643
%#flags: !after before dice offpole UrQMDform stringends
%#V spectrum master v1.4-14-g9842687M
%#dY: 1.000000
%#histogram type: pt
%#flags: after !before dice offpole UrQMDform stringends
%#dpt: 0.500000
%#V histogram master v1.4-14-g9842687M
%#%: hgeos cheos 
%#cascade: 2000, hydro: 1000
%#%: bmeos 
%#V DICE 0x4c2ff8b3
%#events 1866 lines 58104545
%#V DICE 0x4c2ff4eb
%#number of gammas: 9025.936066
%#cascade: 1866, hydro: 933
%#%: cheos 
%#V DICE 0x4c2f78db
%#events 2000 lines 83985497
%#number of gammas: 5618.034379
%#V DICE 0x4c2f736d
%#H pT               bmeos      cascade      ±cascade      cheos        hgeos 
%2.500000e-01 -1.663813e-04 -6.750733e-06 6.460705e-04 -1.011675e-03 -6.313852e-04 
%7.500000e-01 -2.076773e-03 -3.823247e-03 1.363973e-03 -2.812090e-03 -3.619132e-03 
%1.250000e+00 -1.080939e-02 -1.162385e-02 2.708198e-03 -6.021908e-03 -7.301881e-03 
%1.750000e+00 -5.381783e-03 -8.412645e-03 6.387336e-03 -6.533643e-03 -1.053198e-02 
%2.250000e+00  4.362571e-04 -2.844991e-02 1.389391e-02 -1.063046e-03 -8.036721e-03 
%2.750000e+00 -3.866912e-03 -2.988326e-02 3.108235e-02 -1.485244e-02  3.187314e-03 
%3.250000e+00 -2.420830e-02  1.166684e-02 5.074117e-02 -1.468177e-02  2.885887e-02 
% GNUPLOT: LaTeX picture using PSTRICKS macros
% Define new PST objects, if not already defined
\ifx\PSTloaded\undefined
\def\PSTloaded{t}
\psset{arrowsize=.01 3.2 1.4 .3}
\psset{dotsize=.01}
\catcode`@=11

\newpsobject{PST@Border}{psline}{linewidth=.0015,linestyle=solid}
\catcode`@=12

\fi
\psset{unit=5.0in,xunit=\columnwidth,yunit=.9\columnwidth}
\pspicture(0.000000,0.000000)(1.000000,1.000000)
\ifx\nofigs\undefined
\catcode`@=11

\multido{\i=1780000+1117143,\n=0.0+0.5}{8}{
 \PST@Border(0.\i,0.1344) (0.\i,0.1544)
 \PST@Border(0.\i,0.9680) (0.\i,0.9480)
 \rput(0.\i,0.0920){\n}
}
\multido{\i=1344+1389,\ix=-8+2}{7}{
 \PST@Border(0.1780,0.\i)(0.1930,0.\i)
 \PST@Border(0.9600,0.\i)(0.9450,0.\i)
 \rput[r](0.1620,0.\i){\small \ix}
}

\PST@Border(0.1780,0.9679)
(0.1780,0.1344)
(0.9600,0.1344)
(0.9600,0.9679)
(0.1780,0.9679)
\PST@Border(0.1780,0.6901)
(0.9600,0.6901)

\rput{L}(0.0450,0.5511){$v_2^\gamma(p_\bot) [\%]$}
\rput(0.5689,0.0294){x}

\rput[l](0.2950,0.9270){\small Cascade}
\rput[l](0.2950,0.8750){\small HG-EoS}
\rput[l](0.2950,0.8230){\small $\chi$-EoS}
\rput[l](0.2950,0.7710){\small BM-EoS}
\rput[l](0.1900,0.2200){\small U+U @ $E_{\sf lab}=35$~AGeV}
\rput[l](0.1900,0.1700){\small $b < 5$~fm, $|y_{\sf c.m.}| < 0.5$}

\PST@cascl(0.2000,0.9270) (0.2790,0.9270)
\PST@cascl(0.2000,0.9345) (0.2000,0.9195)
\PST@cascl(0.2790,0.9345) (0.2790,0.9195)
\PST@cascd(0.2395,0.9270)
\PST@hgeos(0.2000,0.8750) (0.2790,0.8750)
\PST@xieos(0.2000,0.8230) (0.2790,0.8230)
\PST@bmeos(0.2000,0.7710) (0.2790,0.7710)

\PST@cascl(0.2339,0.6844) (0.2339,0.6934)
\PST@cascl(0.2264,0.6844) (0.2414,0.6844)
\PST@cascl(0.2264,0.6934) (0.2414,0.6934)
\PST@cascl(0.3456,0.6662) (0.3456,0.6851)
\PST@cascl(0.3381,0.6662) (0.3531,0.6662)
\PST@cascl(0.3381,0.6851) (0.3531,0.6851)
\PST@cascl(0.4573,0.5962) (0.4573,0.6338)
\PST@cascl(0.4498,0.5962) (0.4648,0.5962)
\PST@cascl(0.4498,0.6338) (0.4648,0.6338)
\PST@cascl(0.5690,0.6083) (0.5690,0.6971)
\PST@cascl(0.5615,0.6083) (0.5765,0.6083)
\PST@cascl(0.5615,0.6971) (0.5765,0.6971)
\PST@cascl(0.6807,0.5966) (0.6807,0.7896)
\PST@cascl(0.6732,0.5966) (0.6882,0.5966)
\PST@cascl(0.6732,0.7896) (0.6882,0.7896)
\PST@cascl(0.7924,0.4473) (0.7924,0.8791)
\PST@cascl(0.7849,0.4473) (0.7999,0.4473)
\PST@cascl(0.7849,0.8791) (0.7999,0.8791)
\PST@cascl(0.9041,0.1695) (0.9041,0.8744)
\PST@cascl(0.8966,0.1695) (0.9116,0.1695)
\PST@cascl(0.8966,0.8744) (0.9116,0.8744)

\PST@cascd(0.2339,0.6889) (0.3456,0.6756) (0.4573,0.6150) (0.5690,0.6527)
(0.6807,0.6931) (0.7924,0.6632) (0.9041,0.5219)

\PST@hgeos(0.2339,0.6900) (0.3456,0.6635) (0.4573,0.6093) (0.5690,0.6316)
(0.6807,0.4925) (0.7924,0.4825) (0.9041,0.7711)

\PST@xieos(0.2339,0.6857) (0.3456,0.6649) (0.4573,0.6393) (0.5690,0.6169)
(0.6807,0.6342) (0.7924,0.7122) (0.9041,0.8905)

\PST@bmeos(0.2339,0.6830) (0.3456,0.6705) (0.4573,0.6482) (0.5690,0.6447)
(0.6807,0.6827) (0.7924,0.5869) (0.9041,0.5881)

\PST@Border(0.1780,0.9679)
(0.1780,0.1344)
(0.9599,0.1344)
(0.9599,0.9679)
(0.1780,0.9679)

\catcode`@=12
\fi
\endpspicture

